Transport Properties of Anisotropic Polar Fluids:2. Dipolar Interaction

Equilibrium molecular dynamics simulation and the Green-Kubo formalism were used to calculate self-diffusion coefficient, shear viscosity, and thermal conductivity for 38 different dipolar two-center Lennard-Jones fluids along the bubble line and in the homogeneous liquid. It was systematically investigated how anisotropy, i.e. elongation, and dipole momentum influence the transport properties. The reduced elongation L* was varied from 0 to 1 and the reduced squared dipole momentum was varied depending on the elongation as follows: for spherical fluids (L*=0) from $\mu*2=0 to 20, for L*=0.2 from mu*2=0 to 16, and for L*=0.4 and above from mu*2=0 to 12. This represents the entire range in which parameters for real fluids are expected. The statistical uncertainty of the reported data varies with transport property, for self-diffusion coefficient data the error bars are typically lower than 3 %, for shear viscosity and thermal conductivity they are about 8 and 12 %, respectively.

==> bib8_JCP.tex <==
\begin{thebibliography}{99}

\bibitem{fernandez7} G.A. Fern\'{a}ndez, J. Vrabec, and H. Hasse, J. Chem. Phys., submitted (2006).

\bibitem{saager1} B. Saager, R. Hennenberg, and J. Fischer, Fluid Phase Equilibr.  \textbf{71}, 41(1992).

\bibitem{saager2} B. Saager, J. Fischer, Fluid Phase Equillibr.  \textbf{72}, 67(1992).

\bibitem{dubey} G.S. Dubey, S.F. Oshea, and P.A. Monson, Mol. Phys. \textbf{80}, 997(1993).

\bibitem{muller} A. M\"{u}ller, J. Winkelmann, and J. Fischer, J. Chem. Phys. \textbf{99}, 3946(1993).

\bibitem{stoll1} J. Stoll, J. Vrabec, and H. Hasse, Fluid Phase Equilibr. \textbf{209}, 29(2003).

\bibitem{kriebel1} C. Kriebel, A. M\"{u}ller, J. Winkelmann, and
J. Fischer, Mol. Phys. \textbf{87}, 151(1996).

\bibitem{mecke} M. Mecke, J. Fischer, and J. Winkelmann, J. Chem. Phys. \textbf{114}, 5842(2001).

\bibitem{enders} S. Enders, H. Kahl, M. Mecke, and J. Winkelmann, J. Mol. Liq. \textbf{115},
29(2004).

\bibitem{kohler} F. Kohler, N. Van Nhu, Mol. Phys. \textbf{80}, 795(1993).

\bibitem{lisal} M. L\'{i}sal, R. Budinsk\'{y}, V. Vacek, and K. Aim, Int. J. Thermophys. \textbf{20},
163(1999).

\bibitem{kriebel2} C. Kriebel, M. Mecke, J. Winkelmann, J. Vrabec,
and J. Fischer, Fluid Phase Equilibr. \textbf{87}, 151(1996).

\bibitem{stoll2} J. Stoll, J. Vrabec, and H. Hasse, J. Chem. Phys. \textbf{119}, 11396(2003).

\bibitem{vrabec} J. Vrabec, G.K. Kedia, and H. Hasse, Cryogenics \textbf{45}, 253(2005).

\bibitem{vega} C. Vega, B. Saager, J. Fischer, Mol. Phys. \textbf{68}, 1079(1989).

\bibitem{fernandez5} G.A. Fern\'{a}ndez, J. Vrabec, and H. Hasse, Cryogenics, submitted (2006).

\bibitem{lee} S.H. Lee, P.T. Cummings, J. Chem. Phys. \textbf{105}, 2044(1996).

\bibitem{stockmayer} W.H. Stockmayer, J. Chem. Phys. \textbf{9}, 398(1941).

\bibitem{stoll_t} J. Stoll, PhD Thesis, {\it Molecular models for the prediction of thermophysical properties
of pure fluid and mixtures}, Reihe 3, Band 836 (VDI, D\"{u}sseldorf, 2005).

\bibitem{graygubb} C.G. Gray and K.E. Gubbins, {\it Theory of molecular fluids, Vol. 1:
Fundamentals} (Clarendon Press, Oxford, 1984).

\bibitem{lustig} R. Lustig, Mol. Phys. \textbf{65}, 175(1988).

\bibitem{barker} J.A. Barker, R.O. Watts, Mol. Phys. \textbf{26}, 789(1973).

\bibitem{neumann} M. Neumann, O. Steinhauser, Mol. Phys. \textbf{39}, 437(1980).

\bibitem{haile} J.M. Haile, {\it Molecular Dynamics Simulation} (John Wiley \& Sons, New York, 1997).

\bibitem{nose} S. Nos\'{e}, Mol. Phys. \textbf{100}, 191(2002).

\bibitem{frenkel} D. Frenkel, B. Smit. {\it Understandig molecular simulation, from
algoritmus to applications} (Academic Press, San Diego California USA, 2002).

\bibitem{alder3} B.J. Alder, in C. Ciccotti and W.G. Hoover (Ed.), {\it Molecular-dynamic simulation
of statistical-mechanical systems} (North-Holland, Amsterdam, 1986).

\bibitem{alder2} B.J. Alder, D.M. Gass, and T.E. Wainwright, J.
Chem. Phys. \textbf{53}, 3813(1970).

\bibitem{fernandez3} G.A. Fern\'{a}ndez, J. Vrabec, and H. Hasse, Mol. Sim. \textbf{31}, 787(2005).

\bibitem{levesque1} D. Levesque, L. Verlet, and J. K\"{u}rkijarvi, Phys. Rev. A \textbf{7}, 1690(1973).

\bibitem{schoen} M. Schoen and C. Hoheisel, Mol. Phys. \textbf{56}, 653(1985).

\bibitem{erpenbeck2} J.J. Erpenbeck, Phys. Rev. A \textbf{2}, 2514(1974).

\bibitem{fernandezt} G.A. Fern\'{a}ndez, {\it Transport
properties of polar fluids by molecular simulation}, PhD Thesis, University of Stuttgart
(2006).

\bibitem{hansen} J.P. Hansen and I.A. McDonald, {\it Theory of Simple Liquids}
(Academic Press, London, 1986).

%\bibitem{levesque2} D. Levesque and L. Verlet, Phys. Rev. A \textbf{2}, 2514(1970).

%\bibitem{macdowell} L.G. MacDowell, B. Garzon, S. Calero, and S. Lago, J. Chem. Phys. \textbf{106}, 4753 (1997).

%\bibitem{singer} K. Singer, J.V.L. Singer, and A.J. Taylor, Mol. Phys. \textbf{37}, 1239(1979).

%\bibitem{slyusar1} V.P. Slyusar, V.M. Tretyakov, and N.S. Rudenko, Sov. J. Low. Tem. Phys. \textbf{1}, 556(1975).

%\bibitem{slyusar2} V.P. Slyusar, V.M. Tretyakov, and N.S. Rudenko, Sov. J. Low. Tem. Phys. \textbf{4}, 363(1978).

\end{thebibliography}


